Quantum compression with classically simulatable circuits

As we continue to find applications where the currently available noisy devices exhibit an advantage over their classical counterparts, the efficient use of quantum resources is highly desirable. The notion of quantum autoencoders was proposed as a way for the compression of quantum information to reduce resource requirements. Here, we present a strategy to design quantum autoencoders using evolutionary algorithms for transforming quantum information into lower-dimensional representations. We successfully demonstrate the initial applications of the algorithm for compressing different families of quantum states. In particular, we point out that using a restricted gate set in the algorithm allows for efficient simulation of the generated circuits. This approach opens the possibility of using classical logic to find low representations of quantum data, using fewer computational resources.

==> structure.tex <==
%!TEX root = main.tex

%----------------------------------------------------------------------------------------
%	PACKAGES AND OTHER DOCUMENT CONFIGURATIONS
%----------------------------------------------------------------------------------------
% \usepackage{pdfpages}
\usepackage{fancyhdr} % Required for custom headers
\usepackage{lastpage} % Required to determine the last page for the footer
\usepackage{extramarks} % Required for headers and footers
\usepackage{graphicx} % Required to insert images

\usepackage{dcolumn}% Align table columns on decimal point
\usepackage{csquotes}
\usepackage{lipsum} 
\usepackage[english]{babel}
\usepackage[utf8]{inputenc} 
\usepackage[T1]{fontenc}
\usepackage{booktabs}
\usepackage{amssymb}  
\usepackage{amsthm}
\usepackage{amsmath}
\usepackage[makeroom]{cancel}
% \usepackage[dvipsnames]{xcolor}
\usepackage[table,xcdraw]{xcolor}
% \usepackage{bbold}
\usepackage{mathtools}
\usepackage{nameref}
\usepackage{varioref}
\usepackage{hyperref}
\usepackage{cleveref}
\crefname{equation}{Eq.}{Eqs.}
\Crefname{equation}{Equation}{Equations}
\crefname{figure}{Fig.}{Figs.}
\Crefname{figure}{Figure}{Figures}
\crefname{section}{Sect.}{Sects.}
\Crefname{section}{Section}{Sections}
\crefname{table}{Table}{Tables}
\crefname{appsec}{Appendix}{Appendices}
\Crefname{paragraph}{Section}{Sections}
% \usepackage{physics}
\usepackage{qcircuit}
\usepackage{bm}
\usepackage{cite}
\usepackage{footnote}
\usepackage[ruled,vlined]{algorithm2e}
\makesavenoteenv{tabular}
\makesavenoteenv{table}


\usepackage{setspace}
%\singlespacing
%\onehalfspacing
% \doublespacing
%\setstretch{1.1}

\usepackage{geometry}
 \geometry{
 a4paper,
 total={160mm,257mm},
 left=25mm,
 top=20mm,
 }
 
\setlength{\parindent}{2em}
\setlength{\parskip}{0.75em}

\graphicspath{{Figures/}} %Setting the graphicspath

\newcommand{\AC}[1]{\textcolor{red}{[AC: #1]}}
\newcommand{\ac}[1]{\textcolor{red}{#1}}

\newcommand{\abadd}[1]{{\color{MidnightBlue}{#1}}}
\newcommand{\ab}[1]{{\color{RoyalBlue}{[AB: #1]}}}
\newcommand{\red}[1]{{\color[rgb]{0.6,0,0}#1}}


\newcommand{\half}{\frac{1}{2}}
\newcommand{\ket}[1]{| #1 \rangle}
\newcommand{\bra}[1]{\langle #1 |}
\newcommand{\ketbra}[1]{| #1 \rangle\langle #1 |}
\newcommand{\braket}[2]{\langle #1 | #2 \rangle}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}

\newcommand{\expo}[1]{\text{e}^{ #1 }}
\newcommand{\alg}[1]{\textcolor{blue}{#1}}
% \crefname{equation}{Eq.}{Eqs.}
% \Crefname{equation}{Equation}{Equations}
% \crefname{figure}{Fig.}{Figs.}
% \Crefname{figure}{Figure}{Figures}
% \crefname{section}{Sect.}{Sects.}
% \Crefname{section}{Section}{Sections}

\newcommand{\sx}{\hat{\sigma}_x}
\newcommand{\sy}{\hat{\sigma}_y}
\newcommand{\sz}{\hat{\sigma}_z}
\newcommand{\ha}{\hat{a}}
\newcommand{\had}{\hat{a}^\dagger}
\newcommand{\hasq}{\hat{a}^2}
\newcommand{\hadsq}{\hat{a}^{\dagger 2}}
\newcommand{\hXa}{\hat{X}_A}
\newcommand{\hYa}{\hat{Y}_A}
\newcommand{\hy}{\hat{y}}
\newcommand{\hbd}{\hat{b}^\dagger}
\newcommand{\hb}{\hat{b}}
\newcommand{\bb}{\mathbf{b}}
\newcommand{\be}{\mathbf{e}}
\newcommand{\thbd}{\hat{\tilde{b}}^\dagger}
\newcommand{\thb}{\hat{\tilde{b}}}
\newcommand{\hH}{\hat{H}}
\newcommand{\hO}{\hat{\mathcal{O}}}
\newcommand{\hS}{\hat{\mathcal{S}}}
\newcommand{\hE}{\hat{E}}
\newcommand{\hL}{\hat{L}}
\newcommand{\hV}{\hat{V}}
\newcommand{\hT}{\hat{T}}
\newcommand{\hI}{\hat{I}}
\newcommand{\hq}{\hat{q}}
\newcommand{\hQ}{\hat{Q}}
\newcommand{\hN}{\hat{N}}
\newcommand{\hn}{\hat{n}}
\newcommand{\hM}{\hat{M}}
\newcommand{\hK}{\hat{K}}
\newcommand{\hU}{\hat{U}}
\newcommand{\hUd}{\hat{U}^\dagger}
\newcommand{\order}{\mathcal{O}}
\newcommand{\mcL}{\mathcal{L}}

\newcommand{\Hp}{\hH_{\text{prob}}}



\newcommand{\hX}{\hat{X}}
\newcommand{\hY}{\hat{Y}}
\newcommand{\hZ}{\hat{Z}}

\newcommand{\wc}{\omega_r}
\newcommand{\wm}{\omega_m}
\newcommand{\wa}{\omega_a}
\newcommand{\wA}{\omega_A}
\newcommand{\wB}{\omega_B}
\newcommand{\wq}{\omega_q}
\newcommand{\wai}{\omega_{ai}}
\newcommand{\wao}{\omega_{a1}}
\newcommand{\wat}{\omega_{a2}}
\newcommand{\szo}{\hat{\sigma}_{z1}}
\newcommand{\szt}{\hat{\sigma}_{z2}}
\newcommand{\szi}{\hat{\sigma}_{zi}}
\newcommand{\spl}{\hat{\sigma}^{+}}
\newcommand{\sm}{\hat{\sigma}^{-}}
\newcommand{\kA}{\kappa_A}
\newcommand{\kB}{\kappa_B}
\newcommand{\kBe}{\kappa_{B+}}
\newcommand{\kC}{\kappa_C}
\newcommand{\hpsi}{\hat \psi}
\newcommand{\hphi}{\hat \phi}
\newcommand{\hPhi}{\hat \Phi}
\newcommand{\hPhitml}{\hat \Phi_{\text{tml}}}
\newcommand{\Phitml}{\Phi_{\text{tml}}}
\DeclareMathOperator{\trace}{Tr}

% Fermions
\newcommand{\hc}{\hat{c}}
\newcommand{\hcd}{\hat{c}^\dagger}

\newcommand{\lp}{\left(}
\newcommand{\rp}{\right)}
\newcommand{\del}{\partial}

\newcommand{\ie}{\textit{i.e.} }
\newcommand{\eg}{\textit{e.g.} }

\newcommand*{\mathcolor}{}
\def\mathcolor#1#{\mathcoloraux{#1}}
\newcommand*{\mathcoloraux}[3]{%
  \protect\leavevmode
  \begingroup
    \color#1{#2}#3%
  \endgroup
}


\newcommand{\etal}{\textit{et al.}}
